Distance-Aware Private Set Intersection

Private set intersection (PSI) allows two mutually untrusting parties to compute an intersection of their sets, without revealing information about items that are not in the intersection. This work introduces a PSI variant called distance-aware PSI (DA-PSI) for sets whose elements lie in a metric space. DA-PSI returns pairs of items that are within a specified distance threshold of each other. This paper puts forward DA-PSI constructions for two metric spaces: (i) Minkowski distance of order 1 over the set of integers (i.e., for integers $a$ and $b$, their distance is $|a-b|$); and (ii) Hamming distance over the set of binary strings of length $\ell$. In the Minkowski DA-PSI protocol, the communication complexity scales logarithmically in the distance threshold and linearly in the set size. In the Hamming DA-PSI protocol, the communication volume scales quadratically in the distance threshold and is independent of the dimensionality of string length $\ell$. Experimental results with real applications confirm that DA-PSI provides more effective matching at lower cost than naive solutions.

==> HamQueryLite.tex <==
\begin{figure}
	\small
	\begin{mdframed}
		%\begin{protocol}{\AHEthresholdHamQuery: Threshold Hamming Query with AHE}
		
		%\noindent
		
		%\textbf{Inputs:~}  \alice and \bob have vectors $\alicesVector, \bobsVector \in \{0,1\}^{\genericVecLen}$ respectively. and a Hamming distance threshold \hamDistThreshold. 
		
		%\noindent
		%\textbf{Setup:~} \alice and \bob jointly sample \genericVecLen mapping functions \mapSet, \mapDomain 
		%\mapDomain.
		
		\noindent
		\textbf{\underline{Parameters:}} \alice and \bob have vectors $\alicesVector, \bobsVector \in \{0,1\}^{\genericVecLen}$, respectively, and a Hamming distance threshold $\hamDistThreshold \in (0, \genericVecLen/2)$.
		
		
		\smallskip
		\textbf{\underline{Procedure $\mathsf{Map}$}:} 
		
		 \alice and \bob sample \genericVecLen mapping functions \mapSet, \mapDomain. \alice computes set $\alicesSetFromVec \assign \{ s_\setIdx : s_\setIdx \assign \mapSetIdx{\setIdx}(\alicesVector[\setIdx]) \}$. 
		\bob computes $\bobsSetFromVec \assign \{ s_\setIdx : s_\setIdx \assign \mapSetIdx{\setIdx}(\bobsVector[\setIdx]) \}$ \label{step:ham_query_lite:encoding}
	    
		\smallskip
		\textbf{\underline{Procedure \oneSidedSetRecon:}}
		
		\begin{enumerate}[nosep,leftmargin=1.6em,labelwidth=*,align=left]
			
			%\item \alice computes set $\alicesSetFromVec \assign \{a_\setIdx : a_\setIdx \assign \phi_\setIdx(\alicesVector[\setIdx])\}$. 
			%\bob similarly computes $\bobsSetFromVec \assign \{b_\setIdx : b_\setIdx \assign \phi_\setIdx(\bobsVector[\setIdx])\}$ . \label{step:hamQueryLite:encoding}
			
			
			\item \alice encodes \alicesSetFromVec in the polynomial \alicesPoly = \polyFromSet{\alicesSetFromVec} and \bob encodes \bobsSetFromVec in the polynomial \bobsPoly = \polyFromSet{\bobsSetFromVec}. \label{step:set_recon:poly_compute}
			
			
		
			\item \bob samples two degree-\genericVecLen random polynomials $\alicesRandomPoly, \bobsRandomPoly \getsr \polyField$. and a random degree-2\genericVecLen polynomial $\blindingPoly \getsr \polyField$. 
			
			\item For $\ptIdx \in [1, \genericVecLen + 2\hamDistThreshold + 1]$, \alice sends \alicesPolyFromVecEval{x_\ptIdx} to \oleFunc and \bob sends \alicesRandomPolyEval{x_\ptIdx} and \blindingPolyEval{x_\ptIdx}. \alice learns \alicesVoleOutputPolyEval{x_\ptIdx} \assign \blindingPolyEval{x_\ptIdx} + \alicesRandomPolyEval{x_\ptIdx}  \alicesPolyFromVecEval{x_\ptIdx} as the output of \oleFunc. \label{step:set_recon:ole_step_1}
			
			\item For $\ptIdx \in [1, \genericVecLen + 2\hamDistThreshold + 1]$, \bob sends to \alice, \bobsVoleOutputPolyEval{x_\ptIdx} \assign \bobsRandomPolyEval{x_\ptIdx}  \bobsPolyFromVecEval{x_\ptIdx} - \blindingPolyEval{x_\ptIdx}. \label{step:set_recon:ole_step_2}
			
			\item \alice compute set of points \label{step:set_recon:point_computation}
			
			\begin{center}
				$\setOfPtsForInterpolation =  \{(x_\ptIdx, y_\ptIdx) : y_\ptIdx = \frac{\alicesVoleOutputPolyEval{x_\ptIdx} + \bobsVoleOutputPolyEval{x_\ptIdx}}{\alicesPolyFromVecEval{x_\ptIdx}}, ~\ptIdx \in [1, \numPointsForInterpol] \}$.
			\end{center}
			
			\item \alice interpolates \setOfPtsForInterpolation with a rational function $r(x)$ and checks that the denominator of $r(x)$, say $P'(x)$, is a factor of \alicesPoly. If so, \alice outputs $S_A \setminus S_B$ which contains the roots of $P'(x)$, otherwise \alice outputs $\bot$. 	\label{step:set_recon:interpolation}  
			
		\end{enumerate}
		
		\smallskip
		\textbf{\underline{Procedure $\mathsf{Recover}$}:} 
         
         If \alice receives $\bot$ from \oneSidedSetRecon then output $\bot$. Otherwise, upon receiving $\alicesSetFromVec \setminus \bobsSetFromVec$:
		for all  $s_\ptIdx \in \alicesSetFromVec \cap \bobsSetFromVec = \alicesSetFromVec \setminus (\alicesSetFromVec \setminus \bobsSetFromVec)$, let $s_\ptIdx =  \mapSetIdx{\setIdx}(\alicesVector[i])$, then 
		$\bobsVector[i] = \alicesVector[i]$. For all indices $i'$ that are still undetermined , $\bobsVector[i'] = \comp(\alicesVector[i'])$. Output (\alicesVector, \bobsVector).
			


		
		%\begin{enumerate}[nosep,leftmargin=1em,labelwidth=*,align=left]
		
		
	
		%\item \alice and \bob run \oneSidedSetRecon with \alicesSetFromVec and \bobsSetFromVec as inputs respectively. 
		
	

%\end{enumerate}
\end{mdframed}
\vspace{-15pt}
\caption{\small \tHamQueryLite: A first pass Hamming query protocol \label{fig:ham_query_lite}}
\end{figure}


==> SetReconProtocol.tex <==
\begin{figure}
	\small
	\begin{mdframed}
		%\begin{protocol}{\AHEthresholdHamQuery: Threshold Hamming Query with AHE}
		
		\noindent
		\textbf{Inputs:~}  \alice and \bob have set $S_A$ and $S_B$ with \genericVecLen elements, and a set difference threshold \hamDistThreshold. 
		
		\smallskip
		\noindent
		\textbf{Setup:~} \alice and \bob select set of points $\setOfXCoords = \setDefn{\genericVecLen + 2\hamDistThreshold + 1}$ 
		
		\smallskip
		\textbf{Protocol:~}
		
		\begin{enumerate}[nosep,leftmargin=1.6em,labelwidth=*,align=left]
			
			%\item \alice computes set $\alicesSetFromVec \assign \{a_\setIdx : a_\setIdx \assign \phi_\setIdx(\alicesVector[\setIdx])\}$. 
			%\bob similarly computes $\bobsSetFromVec \assign \{b_\setIdx : b_\setIdx \assign \phi_\setIdx(\bobsVector[\setIdx])\}$ . \label{step:hamQueryLite:encoding}
			
			\item \alice encodes $S_A$ in the polynomial \alicesPoly = \polyFromSet{S_A} and \bob encodes $S_B$ in the polynomial \bobsPoly = \polyFromSet{S_B}. \label{step:set_recon:poly_compute}
			
			
			\item \bob samples two degree-\genericVecLen random polynomials $\alicesRandomPoly, \bobsRandomPoly \getsr \polyField$ and a random degree-2\genericVecLen polynomial $\blindingPoly \getsr \polyField$. 
			
			\item For $\ptIdx \in [1, \genericVecLen + 2\hamDistThreshold + 1]$, \alice sends \alicesPolyFromVecEval{x_\ptIdx} to \oleFunc and \bob sends \alicesRandomPolyEval{x_\ptIdx} and \blindingPolyEval{x_\ptIdx}. \alice learns \alicesVoleOutputPolyEval{x_\ptIdx} \assign \blindingPolyEval{x_\ptIdx} + \alicesRandomPolyEval{x_\ptIdx}  \alicesPolyFromVecEval{x_\ptIdx} as the output of \oleFunc. \label{step:set_recon:ole_step_1}
			
			\item For $\ptIdx \in [1, \genericVecLen + 2\hamDistThreshold + 1]$, \bob sends to \alice, \bobsVoleOutputPolyEval{x_\ptIdx} \assign \bobsRandomPolyEval{x_\ptIdx}  \bobsPolyFromVecEval{x_\ptIdx} - \blindingPolyEval{x_\ptIdx}. \label{step:set_recon:ole_step_2}
			
			\item \alice compute set of points \label{step:set_recon:point_computation}
			
			\begin{center}
				$\setOfPtsForInterpolation =  \{(x_\ptIdx, y_\ptIdx) : y_\ptIdx = \frac{\alicesVoleOutputPolyEval{x_\ptIdx} + \bobsVoleOutputPolyEval{x_\ptIdx}}{\alicesPolyFromVecEval{x_\ptIdx}}, ~\ptIdx \in [1, \numPointsForInterpol] \}$.
			\end{center}
			
			\item \alice interpolates \setOfPtsForInterpolation with a rational function $r(x)$ and checks that the denominator of $r(x)$, say $P'(x)$, is a factor of \alicesPoly. If so, \alice outputs $S_A \setminus S_B$ which contains the roots of $P'(x)$, otherwise \alice outputs $\bot$. 	\label{step:set_recon:interpolation}  
			
		\end{enumerate}
		
		%\end{protocol}
	\end{mdframed}
	\vspace{-15pt}
	\caption{\oneSidedSetRecon: Threshold One-Sided Set Reconciliation Protocol. \label{fig:set_recon}}
\end{figure}


==> app_indcpa_claims.tex <==
\subsection{Proof of Claims in Section \ref{sec:tHamQueryfromPSI}}
\label{app:proofClaims}


\indcpaClaimOne*
\begin{proof}
	
	To prove the result, we will show that the probability of obtaining an arbitrary set of $\numPointsForInterpol$ points, 
    in Step 4(b) when $\indcpaBit = 0$, is equal to the probability of obtaining $V$ when $\indcpaBit = 1$. 
	More formally, let $\genericRV_v = \{\genericPt : \genericPtX \in \setOfXCoords, \genericPtY \in \finiteField\}$ be an arbitrary set of $\genericSetSize + 2t + 1$ points. We show that
	
	%To prove the result, we need to show that the probability with which a given set of points $V$ is obtained in Step 5(b), when \indcpaChallengePolyZero is encoded in $r$, is the same as the probability with which $V$ is obtained when \indcpaChallengePolyOne is encoded.  
	
	\begin{center}
		\condProb{V = \genericRV_v}{\indcpaBit = 0} = \condProb{V = \genericRV_v}{\indcpaBit = 1}
	\end{center}
	
	W.l.o.g. let \indcpaBit = 0. Let $U_0(x) = \indcpaChallengePolyZero \alicesRandomPoly + \indcpaFixedPoly \bobsRandomPoly$. From Lemma \ref{lemma:kissener_uniformly_random}, $U_0(x)$ is a uniformly random polynomial of degree $\leq n + D$. For $V = \genericRV_v$, we require for all $x_i \in \setOfXCoords$, 
	$U_0(x_i) = y_i \times P_0(x_i)$ where  $(x_i, y_i) \in \genericRV_v$. There are $\fieldOrder^{\genericSetSize + D + 1}$ polynomials of 
	degree $\leq \genericSetSize + D$.  Out of these, $\fieldOrder^{D - 2t}$ polynomials will pass through the points defined by $\genericRV_v$.  This is because any $\genericSetSize + D + 1$ points uniquely define a polynomial of degree $\leq \genericSetSize + D$. After fixing \setSize{V}  = $\genericSetSize + 2t + 1$ points, we still have $\genericSetSize + D + 1 - (\genericSetSize +2t +1) = D - 2t$ points free.
	Since $U_0(x)$ is uniformly random,
	
	\begin{center}
		\condProb{V = \genericRV_v}{b = 0} = $\frac{\fieldOrder^{D - 2t}}{\fieldOrder^{\genericSetSize + D + 1}} = \fieldOrder^{-(\genericSetSize + 2t + 1)}$
	\end{center}
	
	
	
	Similarly $U_1(x) = \indcpaChallengePolyOne \alicesRandomPoly + \indcpaFixedPoly \bobsRandomPoly$ 
	is a uniformly random polynomial of degree $n + D$ and thus
	for \indcpaBit = 1  
	
	\begin{center}
		\condProb{V = \genericRV_v}{b = 1} = $\fieldOrder^{-(\genericSetSize + 2t + 1)}$
	\end{center}
	
	This completes the proof.
	
	
	% 	Let $r$ = \rationalfn{\indcpaReducedOutputPoly}{\indcpaReducedPoly}
	% 	be the rational function obtained after cancellation of common roots in the numerator and the denominator of  \rationalfn{\indcpaChallengePolyZero \polynomial{R_1} + \indcpaFixedPoly \polynomial{R_2}}{\indcpaChallengePolyZero}.
	% 	From Lemmas \ref{lemma:ghosh_gcd_random} and \ref{lemma:kissener_uniformly_random}, with high probability,  \degree{\indcpaReducedPoly} = $d_0$ since \hamDist{\indcpaFixedVec}{\indcpaChallengeVecZero} =  $d_0$, and \indcpaReducedOutputPoly is a uniformly random polynomial of degree $\leq$ \genericVecLen + $d_0$.
	% 	
	
	% 	For $V = \genericRV_v$, we require \indcpaReducedOutputPolyEval{x_i} = $y_i \times \indcpaReducedPolyEval{x_i}$  for all $(x_i, y_i) \in \genericRV_v$. 
	% 	
	% 	
	% 	\begin{center}
	% 		\condProb{V = \genericRV_v}{b = 0} = $\frac{\fieldOrder^{d_0 - \hamDistThreshold}}{\fieldOrder^{\genericVecLen + d_0 + 1}} = \fieldOrder^{-(\numPointsForInterpol)}$
	% 	\end{center}
	% 	
	
\end{proof}


\indcpaClaimTwo*
\begin{proof}
	
	\indcpaAdversary's winning strategy in this case is to predict $\indcpaAdversaryBit = 0$  if there exists a polynomial of degree $\leq n + D$ passing through all the points $(x_i, y_i \times P_0(x_i))$ for each $(x_i, y_i) \in V$. Similarly, \indcpaAdversary predicts $\indcpaAdversaryBit = 1$ when there exists a polynomial of degree $\leq n + D$ passing through all the points $(x_i, y_i \times P_1(x_i))$ for each $(x_i, y_i) \in V$.
	From Lemma \ref{lemma:twoPolysOnSupSet}, the probability that both these conditions will hold true at the same time $\leq 1/\fieldOrder$. Thus, 
	
	\begin{center}
		\prob{\indcpaAdversaryBit = \indcpaBit} $\geq 1 - 1/\fieldOrder$
	\end{center}
\end{proof}	



==> app_lemma_poly.tex <==

\subsection{Lemmas for Polynomials in \polyField}
\label{app:lemmaPolys}
%\polyOnSupSet*


\begin{restatable}{lemma}{polyOnSupSet}
	\label{lemma:polyOnSupSet}
	Let $X$ be a set of distinct arbitrary values $x_i \in \finiteField$.  
	Let $V$ be a set of random points where each point $v_i = (x_i, y_i), y_i \getsr \finiteField$. Then, the probability that there exists polynomial \polyInField{Q} that satisfies all points in $V$ with $\degree{Q}  \leq D < \setSize{V}$ is $1/\fieldOrder^{\setSize{V} - D - 1}$.
	
\end{restatable}


%\polyOnSupSet*
\begin{proof}
	
	Let $V^{*}$ be the combined set of all sets $V = \{\genericPt : \genericPtX \in \setOfXCoords, \genericPtY \in \finiteField\}$. Then, $|V^{*}| = \fieldOrder^{\setSize{V}}$. Each $V_i \in V^{*}$ is consistent with {\em at most} one polynomial of degree $\leq D$. Otherwise, there will be two or more polynomials of degree $\leq D$ passing through the same \setSize{V} points, which contracts the fact that any $D + 1 \leq \setSize{V}$ points uniquely defines a polynomial of degree $\leq D$
	
	
	Let $P^{*}$ be the set of all polynomials of degree $\leq D$. Clearly, $| P^{*} | =  \fieldOrder^{D+1}$. Each $P_i \in P^{*}$ is consistent with exactly one $V_j \in V^{*}$. Thus, the mapping from $P^{*}$ to $V^{*}$ is injective. Then the probability that $V \in V^{*}$ is satisfied by a polynomial \polyInField{Q} of degree $\degree{Q} \leq D$ is given by the probability that $V$ has a pre-image in the injective map which is $1/\fieldOrder^{\setSize{V} - D - 1}$.
\end{proof}

	
%Also note that there are exactly $\fieldOrder^{D+1}$ polynomials of degree $\leq D$. Each such polynomial is consistent with exactly one unique set of points of size \setSize{V}. 

%Thus, there exists an injective map from polynomials of degree $\leq D$ to the sets of size \setSize{V} comprising points that lie on the corresponding polynomials. 


%\twoPolysOnSupSet*

% 


\iffalse
\begin{restatable}{lem}{twoPolysOnSupSet}
	\label{lemma:twoPolysOnSupSet}
	Let $U_{0}(x)$ be a random polynomial of degree $D$ and let $P_0(x)$ and $P_1(x)$ be two fixed 
	polynomials of degree $\leq \degree{U_0(x)}$. Let $\setOfXCoords = \setOfXCoordsDefn$ be an arbitrary set of values in $\finiteField$, and $V = \{\genericPt : \genericPtX \in \setOfXCoords, \genericPtY \in \finiteField\}, \setSize{V} > D+1$ be a set of points that lie on the rational function \rationalfn{U_0(x)}{P_0(x)}. Then the probability that there exists a polynomial $U_{1}(x)$ of degree $D$ such that the rational 
	function $\rationalfn{U_1(x)}{P_1(x)}$ is consistent with all points in $V$ is $\leq 1/\fieldOrder$.
	%  such that for each point $v_i = (x_i, y_i \times P_0(x_i))$ in $V$, the point $v_i = (x_i, y_i \times P_1(x_i))$ lies on $U_1(x)$ is 
\end{restatable}

\begin{proof}
	
	Note that the required condition holds iff. $\forall \genericPt \in V$, 
	
	\begin{center}
		$U_1(\genericPtX) = U_0(\genericPtX) \times \frac{P_1(\genericPtX)}{P_0(\genericPtX)}$
	\end{center}
	
	That is $U_1(x)$ is consistent with the set of points $V' = \{\genericPt : \genericPtY = U_0(\genericPtX) \times \frac{P_1(\genericPtX)}{P_0(\genericPtX)}\}$. 
	Since $U_0(x)$ is a random polynomial, the $y_i$'s are random. From Lemma \ref{lemma:polyOnSupportSet}, the probability that there exists a polynomial of degree $D$ consistent with $V'$ is $\fieldOrder^{-(|V| - D - 1)} \leq 1/p$.	
	
	%	First note that for any random polynomial $U_{0}(x)$ of degree $D$,  $U_{0}(x) P_1(x) - U_{1}(x) P_0(x)$ is a uniformly random polynomial of degree from Lemma \ref{lemma:kissener_uniformly_random}. For the result, we require for all $x_i \in \setOfXCoords$: 
	%	
	%	\begin{center}
	%		$U_{0}(x_i) P_1(x_i) - U_{1}(x_i) P_0(x_i) = 0$
	%	\end{center}
	%	
	%	That is, the polynomial $U_{0}(x_i) P_1(x_i) - U_{1}(x_i) P_0(x_i) = 0$ has roots at all the values in \setOfXCoords.
	%	This happens with probability $\fieldOrder^{-|V|}$. There are $(\fieldOrder - 1)\times \fieldOrder^{D}$ polynomials of degree $D$ in \polyField. The probability that at least one of these polynomials yields a polynomial $U_{0}(x) P_1(x) - U_{1}(x) P_0(x)$ with roots at all values in \setOfXCoords is $\leq 1/\fieldOrder$
	
\end{proof}	
\fi

==> app_security_ham_psi.tex <==
\section{Proofs for Section \ref{sec:hamming awarePSI}}


==> app_security_ham_query.tex <==
\section{Proofs}

\subsection{Proof of Fact~\ref{fact:hamming_dist_compute}}
\label{app:proof_hamming_compute}
\hammingCompute*
\begin{proof}
	Let $S_{01} = \{m \in [1, \genericVecLen] ~:~ \alicesVector[m] = 0, \bobsVector[m] = 1\}$, $S_{10} = \{m \in [1, \genericVecLen] ~:~ \alicesVector[m] = 1, \bobsVector[m] = 0\}$ and $S_{11} = \{m \in [1, \genericVecLen] ~:~ \alicesVector[m] = 1, \bobsVector[m] = 1\}$. Then, 
	
	\begin{center}
		$\hamWeight{\alicesVector} = \setSize{S_{10}} + \setSize{S_{11}}$ \\
		$\hamWeight{\bobsVector} = \setSize{S_{01}} + \setSize{S_{11}}$ \\
		$\hamDist{\alicesVector}{\bobsVector} = \setSize{S_{10}} + \setSize{S_{01}}$
	\end{center}
	
	The above equations along with the fact $\setSize{S_{11}} = \sum\limits_{m = 1}^{\genericVecLen} \alicesVector[m] \cdot \bobsVector[m]$ proves the result. 
\end{proof}

\subsection{Proof of Fact~\ref{fact:balls_bins_2}}
\label{app:proof_balls_bins}
\ballsbins*
\begin{proof}
	Let $E_k$ be the event that there are $\numOfBins - (2\hamDistThreshold + 1 - k)$ empty bins i.e., only $(2\hamDistThreshold  + 1 - k)$ bins are non-empty where $k \in [2, 2\hamDistThreshold - 1)$. Then,

	\begin{center}
		$\prob{E_k} = \frac{(2\hamDistThreshold + 1 - k)! \stirling{2\hamDistThreshold+1}{2\hamDistThreshold + 1 - k} \binom{\numOfBins}{\numOfBins - (2\hamDistThreshold + 1- k)}}{(\numOfBins)^{2\hamDistThreshold+1}}$ \\
		
		$ = \frac{(2\hamDistThreshold)! \stirling{2\hamDistThreshold+1}{2\hamDistThreshold + 1 - k} \binom{\numOfBins}{2\hamDistThreshold + 1 - k}}{(\numOfBins)^{2\hamDistThreshold+1}}$
		
		$ \leq \stirling{2\hamDistThreshold+1}{2\hamDistThreshold + 1 - k} \times \left(\numOfBinsFrac\right)^{-k}$ 
		
	\end{center}
	
	where $\stirling{a}{b}$ denotes the Stirling number of the second kind. Also, $\stirling{a}{b} \leq \frac{1}{2} \binom{a}{b} b^{a - b}$. Thus, we find, 
	
	\begin{center}
		$\stirling{2\hamDistThreshold+1}{2\hamDistThreshold + 1 - k}  \leq \frac{1}{2} \binom{2\hamDistThreshold+1}{2\hamDistThreshold + 1 - k} (2\hamDistThreshold + 1 - k)^{k} \leq \frac{1}{2} \frac{(2\hamDistThreshold + 1)^{k} (2\hamDistThreshold + 1 - k)^{k}}{k!} $
		
	\end{center}
	
	Now, $\frac{(2\hamDistThreshold + 1) (2\hamDistThreshold + 1 - k)}{\numOfBins} < 1.5\epsilon$. Thus, 
	
	\begin{center}
		$\prob{E_k} < \frac{1}{2} \times \epsilon^k \times \frac{1.5^k}{k!}$
		
	\end{center}
	
	Let $E$ be the event that the number of empty bins $ \geq \numOfBins - 2\hamDistThreshold + 1$. Then, 
	
	
	\begin{center}
		$\prob{E} \leq \sum\limits_{k = 2}^{2\hamDistThreshold - 2} \prob{E_k} = \sum\limits_{k = 2}^{2\hamDistThreshold - 2} \frac{1}{2} \times \epsilon^k \times \frac{1.5^k}{k!} < \frac{\epsilon}{2} \times \left(\sum\limits_{k = 2}^{2\hamDistThreshold - 2} \frac{1.5^k}{k!}\right) < \epsilon$
	\end{center}
	
	Note that the last two inequalities hold since $\epsilon \in (0,1)$ and $\sum\limits_{k = 2}^{\infty} \frac{1.5^k}{k!} = e^{1.5} - 2.5 \approx 1.9$. 
\end{proof}


==> document.tex <==
\section{Evaluation}

==> plot_hamPSI.tex <==
\pgfplotscreateplotcyclelist{grayscale}{
	very thick,white!10!black,mark=o,mark options={scale=1.5},solid,densely dotted\\%
	very thick,white!20!black,mark=x,mark options={scale=1.5}, solid,densely dotted\\%
	very thick,white!30!black,mark=*,mark options={scale=1.5}, solid,densely dotted\\%
	very thick,white!40!black,mark=+,mark options={scale=1.5}, solid,dashed\\%
	very thick,white!50!black,mark=x,mark options={scale=1.5}, solid,dashed\\%
}



\begin{figure}[ht!]
	\centering
		\begin{tikzpicture}[scale=0.5]
		\begin{axis}[
		cycle list name=grayscale,
		xlabel=Distance Threshold,
		ylabel=Total Comm. (in GB.),
		ymax=5
		]
	
	
	\addplot+[line width=2.5pt, white!50!black, solid] coordinates {(1, 3) (2, 3.1)  (4, 3.1) (6, 3.1) (8, 3.2) (10, 3.2) (12, 3.2) (14, 3.2) (16,3.2) (18,3.2)(20,3.2)};
	\addplot+[line width=2.5pt, white!10!black, solid] coordinates {(1, .009) (2, .027) (4, .089) (6, .185) (8, .315)
	(10, .479) (12, .678) (14, .9) (16, 1.1) (18, 1.4 ) (20, 1.8)};
	\legend{GC Baseline, \hamAwarePSIProtocol}

		
		\end{axis}
		\end{tikzpicture}
	
\vspace{-8pt}
\caption{Application benchmark for \hamAwarePSIProtocol. With sets of size 100 comprising 6000-bit vectors representing iris images, the communication volume is $1.8\times$ lower for \hamAwarePSIProtocol compared to the GC-baseline with a distance threshold of $20$.  \label{fig:hamPSI:app:comm_threshold}
} 
\end{figure}


==> plot_intPSI_app.tex <==
\pgfplotscreateplotcyclelist{grayscale}{
	very thick,white!10!black,mark=o,mark options={scale=1.5},solid,densely dotted\\%
	very thick,white!20!black,mark=x,mark options={scale=1.5}, solid,densely dotted\\%
	very thick,white!30!black,mark=*,mark options={scale=1.5}, solid,densely dotted\\%
	very thick,white!40!black,mark=+,mark options={scale=1.5}, solid,dashed\\%
	very thick,white!50!black,mark=x,mark options={scale=1.5}, solid,dashed\\%
}

\begin{figure}
	\centering
	\subfloat[Comm vs. threshold]
	{ \label{fig:intPSI:macro:comm_threshold}
		\begin{tikzpicture}[scale=0.5]
			\begin{axis}[
				cycle list name=grayscale,
				legend pos = north west,
				xlabel=Distance Threshold,
				ylabel=Total Comm. (in MB.)
				]
				\addplot coordinates {(0,1.9) (2,3.6) (4,7.2) (8,13.2) (16,24.7) (32,30) (64,39) (128,46) };
				%\addlegendentry{\sysname~}
				\addplot coordinates {(0,1.9) (2,9.7) (4,17.4) (8,32.4) (16,62.4) (32,130) (64,250) (128,434)};
				%\addlegendentry{\sysname~}
				\legend{\intAwarePSIProtocol, DA Baseline}
				
			\end{axis}
		\end{tikzpicture}
	}
	\subfloat[Compute time vs. threshold]
	{\label{fig:intPSI:macro:comp_threshold}
		\begin{tikzpicture}[scale=0.5]
			\begin{axis}[
				ybar = 0pt,
				enlargelimits=0.15,
				bar width = 0.2cm,
				xlabel=Distance Threshold,
				ylabel={Time (in ms, log scale)},
				legend pos = north west,
				symbolic x coords={0, 2, 4, 8, 16, 32, 64, 128},
				%nodes near coords,
				%nodes near coords align={horizontal},
				cycle list = {black,black!70,black!40,black!10}
				]
				\addplot+[] coordinates {(0, 2.4 ) (2, 2.5) (4,2.6) (8, 2.7) (16, 2.9) (32,3) (64,3.11) (128,3.17)};
				\addplot+[fill,text=black] coordinates {(0, 2.4) (2, 2.6) (4,2.7) (8,2.9) (16,3.2) (32,3.5) (64,3.8) (128,4.1)};
				\legend{\intAwarePSIProtocol, DA Baseline}
			\end{axis}
	\end{tikzpicture}}
	\vspace{-15pt}
	\caption{\small Benchmarks for \intAwarePSIProtocol applied to private collaborative blacklisting. Set size = 25k. The communication volume and compute time for \intAwarePSIProtocol are both around $\mathbf{10\times}$ less than the baseline when threshold = 128.}
\end{figure}

==> proofs_hamming.tex <==
\section{Proofs}

\subsection{Proof of \propref{claim:}}


\subsection{Proof of Fact~\ref{fact:hamming_dist_compute}}
\label{app:proof_hamming_compute}
\hammingCompute*
\begin{proof}
	Let $S_{01} = \{m \in [1, \genericVecLen] ~:~ \alicesVector[m] = 0, \bobsVector[m] = 1\}$, $S_{10} = \{m \in [1, \genericVecLen] ~:~ \alicesVector[m] = 1, \bobsVector[m] = 0\}$ and $S_{11} = \{m \in [1, \genericVecLen] ~:~ \alicesVector[m] = 1, \bobsVector[m] = 1\}$. Then, 
	
	\begin{center}
		$\hamWeight{\alicesVector} = \setSize{S_{10}} + \setSize{S_{11}}$ \\
		$\hamWeight{\bobsVector} = \setSize{S_{01}} + \setSize{S_{11}}$ \\
		$\hamDist{\alicesVector}{\bobsVector} = \setSize{S_{10}} + \setSize{S_{01}}$
	\end{center}
	
	The above equations along with the fact $\setSize{S_{11}} = \sum\limits_{m = 1}^{\genericVecLen} \alicesVector[m] \cdot \bobsVector[m]$ proves the result. 
\end{proof}

\subsection{Proof of Fact~\ref{fact:balls_bins_2}}
\label{app:proof_balls_bins}
\ballsbins*
\begin{proof}
	Let $E_k$ be the event that there are $\numOfBins - (2\hamDistThreshold + 1 - k)$ empty bins i.e., only $(2\hamDistThreshold  + 1 - k)$ bins are non-empty where $k \in [2, 2\hamDistThreshold - 1)$. Then,
	
	
	
	\begin{center}
		$\prob{E_k} = \frac{(2\hamDistThreshold + 1 - k)! \stirling{2\hamDistThreshold+1}{2\hamDistThreshold + 1 - k} \binom{\numOfBins}{\numOfBins - (2\hamDistThreshold + 1- k)}}{(\numOfBins)^{2\hamDistThreshold+1}}$ \\
		
		$ = \frac{(2\hamDistThreshold)! \stirling{2\hamDistThreshold+1}{2\hamDistThreshold + 1 - k} \binom{\numOfBins}{2\hamDistThreshold + 1 - k}}{(\numOfBins)^{2\hamDistThreshold+1}}$
		
		$ \leq \stirling{2\hamDistThreshold+1}{2\hamDistThreshold + 1 - k} \times \left(\numOfBinsFrac\right)^{-k}$ 
		
	\end{center}
	
	where $\stirling{a}{b}$ denotes the Stirling number of the second kind. Also, $\stirling{a}{b} \leq \frac{1}{2} \binom{a}{b} b^{a - b}$. Thus, we find, 
	
	\begin{center}
		$\stirling{2\hamDistThreshold+1}{2\hamDistThreshold + 1 - k}  \leq \frac{1}{2} \binom{2\hamDistThreshold+1}{2\hamDistThreshold + 1 - k} (2\hamDistThreshold + 1 - k)^{k} \leq \frac{1}{2} \frac{(2\hamDistThreshold + 1)^{k} (2\hamDistThreshold + 1 - k)^{k}}{k!} $
		
	\end{center}
	
	Now, $\frac{(2\hamDistThreshold + 1) (2\hamDistThreshold + 1 - k)}{\numOfBins} < 1.5\epsilon$. Thus, 
	
	\begin{center}
		$\prob{E_k} < \frac{1}{2} \times \epsilon^k \times \frac{1.5^k}{k!}$
		
	\end{center}
	
	Let $E$ be the event that the number of empty bins $ \geq \numOfBins - 2\hamDistThreshold + 1$. Then, 
	
	
	\begin{center}
		$\prob{E} \leq \sum\limits_{k = 2}^{2\hamDistThreshold - 2} \prob{E_k} = \sum\limits_{k = 2}^{2\hamDistThreshold - 2} \frac{1}{2} \times \epsilon^k \times \frac{1.5^k}{k!} < \frac{\epsilon}{2} \times \left(\sum\limits_{k = 2}^{2\hamDistThreshold - 2} \frac{1.5^k}{k!}\right) < \epsilon$
	\end{center}
	
	Note that the last two inequalities hold since $\epsilon \in (0,1)$ and $\sum\limits_{k = 2}^{\infty} \frac{1.5^k}{k!} = e^{1.5} - 2.5 \approx 1.9$. 
\end{proof}

